Linearising Explicit Substitutions using Intersection Types

Term expansion was originally introduced in 2004 as a way to relate terms typed in an intersection type system with linear terms. Recently, new applications of term expansion include the relation of lambda-terms with terms typed in other substructural type systems, such as the relevant and the ordered type systems, and the use of quantitative types to relate the strongly normalising lambda-terms with weak linear terms that share the same normal form. Here we define a new term expansion for a calculus with explicit substitutions, using it to relate a lambda-calculus with explicit substitutions to Boudol's resource aware lambda-calculus with multiplicities, where function arguments have a possibly limited availability.

==> eptcsdata.tex <==
\providecommand{\firstpage}{19}
\providecommand{\publicationstatus}{V. de Paiva; T.A. de Lima (Eds.): 21st International Symposium\\ on Logical and Semantic Frameworks, with Applications (LSFA 2026)\\
EPTCS 449, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.449.2}{10.4204/EPTCS.449.2}}

